ARKit LabelMaker: A New Scale for Indoor 3D Scene Understanding

Neural network performance scales with both model size and data volume, as shown in both language and image processing. This requires scaling-friendly architectures and large datasets. While transformers have been adapted for 3D vision, a `GPT-moment' remains elusive due to limited training data. We introduce ARKit LabelMaker, a large-scale real-world 3D dataset with dense semantic annotation that is more than three times larger than prior largest dataset. Specifically, we extend ARKitScenes with automatically generated dense 3D labels using an extended LabelMaker pipeline, tailored for large-scale pre-training. Training on our dataset improves accuracy across architectures, achieving state-of-the-art 3D semantic segmentation scores on ScanNet and ScanNet200, with notable gains on tail classes. Our code is available at https://labelmaker.org and our dataset at https://huggingface.co/datasets/labelmaker/arkit_labelmaker.

==> workshop_sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Large-scale deep learning has achieved remarkable success in language models \cite{radford2018gpt1,radford2019gpt2,brown2020gpt3} and 2D vision \cite{radford2021learning,rombach2022stablediffusion,achiam2023gpt} by leveraging web-scale unlabeled data. However, this approach is not directly applicable to 3D scene understanding, where real-world 3D data lacks web-scale abundance and demands labor-intensive ground truth annotations. While recent work explores semi-supervised \cite{jiang2023selfsupervised-pretraining,zhu2023ponderv2} and open-set \cite{ovseg, wu2024ptv3, yilmaz2024opendas, takmaz2025search3d, engelmann2024opennerf} methods to reduce labeling effort, state-of-the-art 3D segmentation~\cite{wu2024ptv3, nekrasov2021mix3d, mask3d, yue2023agile3d} remains dependent on curated datasets orders of magnitude smaller than those in other modalities. This makes large-scale 3D dataset construction a significant need.

In this paper, we improve an automatic labeling pipeline to create the largest real-world 3D indoor dataset. Our work investigates the following research question \emph{``Does large-scale pre-training with automatic labels show similar trends as it does for language and image generation tasks?"} through the following key contributions:
\begin{itemize}[leftmargin=*]
    \item We enhance LabelMaker~\cite{labelmaker} to LabelMakerV2 with updated base models (Grounded-SAM), gravity alignment correction, and mobile app integration.
     \item We apply LabelMakerV2 to ARKitScenes~\cite{baruch2021arkitscenes}, and generate the largest existing real-world 3D dataset, \textbf{ARKit LabelMaker}, with dense semantic annotations on 186 classes using 48'000 GPU hours on Nvidia 3090 GPUs. 
     \item With ARKit LabelMaker dataset, we improve over state-of-the-art PointTransformer on ScanNet200 by 2.1\%, on tail classes by 5.5\% mIoU.
     \item We analyze the trade-off between training in unsupervised settings, on synthetic data, and on auto-labeled real-world data, guiding future data scaling efforts.
\end{itemize}

% teaser figure
\input{table_and_figure_tex/fig_1_teaser.tex}

==> workshop_sec/2_related_works.tex <==
\section{Related Works}
\label{sec:related_works}

\paragraph{Datasets for 3D semantic segmentation.}
% table dataset scale
\input{table_and_figure_tex/tab_1_datasets_scale.tex}

\paragraph{3D semantic segmentation models.}

\paragraph{LabelMaker}~\cite{labelmaker} is an automated semantic annotation pipeline that generates unified 2D and 3D labels by aggregating outputs from diverse segmentation models. The method processes RGB-D video frames using an ensemble of state-of-the-art 2D and 3D segmentation models trained on heterogeneous label spaces. LabelMaker resolves semantic discrepancies between these models by mapping all predictions to a unified label space using \emph{wordnet synkeys}~\cite{wordnet}, denoted as the WordNet label space. The pipeline then performs two-stage refinement: (1) per-frame consensus generation through model prediction aggregation, followed by (2) label lifting into 3D point clouds where multi-view consistency is enforced via per-point voting across frames. The output includes coherent 3D semantic annotations for point clouds and back projected 2D labels for image-based segmentation tasks.

==> workshop_sec/3_method.tex <==
\section{Method}
\label{sec:method}

% pipeline figure
\input{table_and_figure_tex/fig_2_labelmaker_pipeline.tex}

We enhance LabelMaker through three principal modifications: (1) integrating open-vocabulary segmentation capabilities, (2) enforcing gravity-aware image alignment, and (3) enabling mobile capture processing. Figure~\ref{fig:pipeline-task-dependency} illustrates the enhanced workflow.

\paragraph{Grounded-SAM Integration.} We enhance LabelMaker with Grounded-SAM~\cite{liu2023grounding} as an additional vote in the ensemble. G-SAM combines two complementary models, Grounding DINO~\cite{liu2023grounding} which detects object bounding boxes using semantic labels, and Segment Anything (SAM)~\cite{kirillov2023segment} generates high quality masks for these regions. This integration addresses LabelMaker's original limitation of excluding SAM's segmentation capabilities, which generalize robustly to novel environments. To align with LabelMaker's unified label space, we adapt Grounding DINO's original label space to our WordNet label space.

\paragraph{Gravity Alignment.} Semantic segmentation models achieve optimal performance when input images align with the gravity direction assumed during training. However, mobile captures from datasets like ARKitScenes frequently contain rotated frames due to device orientation changes during scanning. These rotations cause severe misclassifications in LabelMaker's base models, particularly confusing gravity-dependent classes like floors and ceilings. We resolve this by leveraging ARKit's inertial measurement unit (IMU) data to estimate the sky direction vector.  For each frame, we compute the angular offset $\alpha$ between the camera's upward direction and the sky vector. The image is then rotated by $k\cdot \frac{\pi}{2}$, where integer $k = \arg \min_{s}(|s\frac{\pi}{2} - \alpha|)$, ensuring near-upright orientation for segmentation inference. Final predictions are inversely rotated to match the original coordinate system before label fusion.

\paragraph{Omission of NeuS.} LabelMaker optionally employed NeuS~\cite{wang2021neus}, an implicit neural surface model with a semantic head for 3D lifting and 2D denoising. We omit this step due to two critical limitations. First, NeuS requires per-scene optimization, incurring prohibitive computational costs. Second, NeuS optimizes its own geometry of the scene that in ‘inside-out’ scans of ARKitScenes is not well constrained. Hense, we kept per-point voting from \cite{labelmaker} as it was the most stable in our initial exploration.

\paragraph{Mobile Integration.}
We integrate LabelMaker with the iOS app Scanner 3D to process consumer-grade RGB-D captures from mobile devices. This enables direct ingestion of smartphone scans into the annotation pipeline, eliminating the need for specialized dataset collection setups. Users can now generate semantic labels for arbitrary scenes captured with everyday devices.

==> workshop_sec/4_results.tex <==
\section{Results}
\label{sec:results}

\todo{introducing baseline models and dataset used, also introduce training paradigm, metric}.


\subsection{Experiments}

% scannet 200 results
\input{table_and_figure_tex/tab_2_scannet200.tex}

% scannet results
\input{table_and_figure_tex/tab_3_scannet.tex}

% table: ARKit LabelMaker percentage scaling and synthetic dataset
\input{table_and_figure_tex/tab_4_alc_percentage_scaling.tex}


